Locality-sensitive hashing of curves

We study data structures for storing a set of polygonal curves in ${\rm R}^d$ such that, given a query curve, we can efficiently retrieve similar curves from the set, where similarity is measured using the discrete Fr\'echet distance or the dynamic time warping distance. To this end we devise the first locality-sensitive hashing schemes for these distance measures. A major challenge is posed by the fact that these distance measures internally optimize the alignment between the curves. We give solutions for different types of alignments including constrained and unconstrained versions. For unconstrained alignments, we improve over a result by Indyk from 2002 for short curves. Let $n$ be the number of input curves and let $m$ be the maximum complexity of a curve in the input. In the particular case where $m \leq \frac{\alpha}{4d} \log n$, for some fixed $\alpha>0$, our solutions imply an approximate near-neighbor data structure for the discrete Fr\'echet distance that uses space in $O(n^{1+\alpha}\log n)$ and achieves query time in $O(n^{\alpha}\log^2 n)$ and constant approximation factor. Furthermore, our solutions provide a trade-off between approximation quality and computational performance: for any parameter $k \in [m]$, we can give a data structure that uses space in $O(2^{2k}m^{k-1} n \log n + nm)$, answers queries in $O( 2^{2k} m^{k}\log n)$ time and achieves approximation factor in $O(m/k)$.

==> constrains.tex <==


\subsection{LSH for anchored distances}
\seclab{anchored}
\input{lsh_anchored}

\subsection{LSH for bounded-speed distances}
\seclab{speed}
\input{lsh_speed}	

==> extension.tex <==
\seclab{basic:continuous:all}
In this section we extend the basic LSH scheme to the continuous \Frechet
distance for curves on the real line.  This classical version of the \Frechet
distance measures similarity between polygonal curves using continuous
bijections between the curves.  We will obtain an LSH with the same bounds as
in the case of the discrete \Frechet distance.  We start by giving the classical
definition of the \Frechet distance for curves in $\Re^d$. For the remainder of
the section we will only consider curves on the real line.

\begin{definition}
Let $\mathcal W$ denote the set of continuous and increasing functions
$f:[0,1]\rightarrow[0,1]$ with the property that $f(0)=0$ and $f(1)=1$. 
For two given curves 
$P:[0,1]\rightarrow \Re^d$ and $Q:[0,1]\rightarrow \Re^d$,
their \emph{\Frechet distance} is defined as 
\begin{equation*} \label{def:frechet} 
\distFr{P}{Q}=\inf_{f\in \mathcal W}\; \max_{t \in [0,1]} \| P(f(t))-Q(t)
\|.
\end{equation*}
\end{definition}

\subsection{Algorithm}
\seclab{basic:continuous}

Let $P:[0,1]\rightarrow \Re$ be a polygonal curve on the real line defined by
vertices $p_1,\dots,p_m \in \Re$.  We extend the basic LSH scheme described in
\secref{basic} as follows.  In the first step we apply the same hash function
as before, namely we snap the vertices of $P$ to a randomly shifted grid of
size $\delta$.  The grid is shifted by a parameter $t \in [0,1)$.   In a second
step, we remove all vertices that lie on the line segment connecting their
adjacent vertices.  That is, $p_i$ is removed iff either $p_i \in
[p_{i-1},p_{i+1}]$ or  $p_i \in [p_{i+1},p_{i-1}]$.  As before, the second step
ensures that two curves with zero \Frechet distance after the snapping will
also have the exact same sequence of vertices.  We denote with $\Hash_{\delta}$
be the family of hash functions $h^t_{\delta}$ constructed this way, where $t$
is distributed uniformly random in $[0,1)^d$.


\subsection{Signatures}

To prove that the above scheme yields the claimed bounds, we use the concept 
of signatures previously introduced by Driemel, Krivo\v{s}ija and Sohler in
\cite{dks-clust-16}.  
A signature is a specific from of curve simplification, that can be obtained by
edge-contractions. Consider contracting the edges of a curve $P$ in the order of their
length, beginning with the shortest edge\footnote{For technical reasons we make
an exception for the edges connected to the first vertex and the last vertex of
the curve. These edges are only contracted if their length is shorter than half
of any of the inner edges. Furthermore, a contraction of such an edge keeps the
first, respectively the last vertex of the curve intact. For details refer to
\cite{dks-clust-16}.}, and consider the sequence of curves that is obtained by
this operation. It can be
seen that the sequences of edge lengths of the contracted edges is
monontonically decreasing.  Let $\ell_i$ be the length of the $i$-th contracted
edge and let $S_i$ be the resulting curve. We call $S_i$ the $\gamma$-signature 
of $P$ for any $\gamma \in (\ell_i,\ell_{i+1}]$.

As shown in \cite{dks-clust-16}, the set of signatures obtained by the above 
edge-contracting procedure can alternatively be defined as follows. The formal 
definition also reveals some useful properties.

\begin{definition}[$\delta$-signature]\deflab{signature}
We define the $\delta$-signature of any curve $P: [0,1]\rightarrow
\Re$ as follows.
The signature is a curve $A: [0,1] \rightarrow \Re$ defined by a series of
values $0=t_1 <\dots<t_m=1$ as the linear interpolation of $P(t_i)$ in the
order of the index $i$, and with the following properties.\\ For $1 \leq i \leq
m -1$ the following conditions hold: 
\begin{compactenum}[(i)]
\item (non-degeneracy) if $i \in [2,m-1]$ then $P(t_i) \notin \langle P(t_{i-1}), P(t_{i+1})\rangle $,
\item (direction-preserving)\\if $P(t_i)<P(t_{i+1})$ for $t < t' \in [t_i,t_{i+1}]$:
$P(t)-P(t') \leq 2\delta$, and \\if $P(t_i)>P(t_{i+1})$ for $t < t'
\in [t_i,t_{i+1}]$: $P(t')-P(t) \leq 2\delta$,
\item (minimum edge length)\\if $i \in [2,m-2]$ then $|P(t_{i+1})-P(t_i)| > 2\delta$, and \\if
$i\in \{1,m-1\}$ then $|P(t_{i+1})-P(t_{i})| > \delta$,
\item (range) for $t \in [t_i,t_{i+1}]$: \\if 
$i \in [2,m-2]$ then $P(t) \in \langle P(t_i), P(t_{i+1})\rangle$, and \\if 
$i=1$ and $m>2$ then $P(t) \in \langle P(t_i),P(t_{i+1})\rangle \cup \langle
P(t_i)-\delta,P(t_i)+\delta\rangle$, and \\if 
$i=m -1$  and $m>2$ then $P(t) \in \langle P(t_{i-1}),P(t_i)\rangle \cup \langle
P(t_i)-\delta,P(t_i)+\delta\rangle$, and \\if
$i=1$ and $m=2$ then $P(t) \in \langle P(t_{1}),P(t_2)\rangle \cup \langle
P(t_1)-\delta,P(t_1)+\delta\rangle \cup \langle
P(t_2)-\delta,P(t_2)+\delta\rangle.$
\end{compactenum}
\end{definition}

%It was established in \cite{dks-clust-16} that for any curve $P$
%its $\gamma$-signature  can be computed in $O(m)$ time for any $\gamma \geq 0$. 
We have the following fact, which will be used in the proof of \lemref{cfd:a1}. 

%\begin{fact}\factlab{fd:signature}{\cite{dks-clust-16}}
%For any curve $P$ and any $\delta>0$, let $S$ be the $\delta$-signature of $P$. 
%It holds that $\distFr{P}{S}\leq \delta$.
%\end{fact}
%
%\begin{fact}\factlab{canonical:signature}
%Given a polygonal curve $P:[0,1]\rightarrow\Re$ with vertices in general position, there exists a
%series of signatures $A_1,A_2,\dots,A_k$ and corresponding parameters
%$0 = \delta_1 < \delta_2 < \dots < \delta_{k+1}$, such that 
%\begin{compactenum}[(i)]
%\item $A_i$ is a %minimal 
%$\delta$-signature of $P$ for any $\delta \in [\delta_i,\delta_{i+1})$, 
%\item the vertex set of $A_{i+1}$ is a subset of the vertex set of $A_{i}$,
%\item $A_k$ is the linear interpolation of $P(0)$ and $P(1)$.
%\end{compactenum}
%\end{fact}
%
\begin{fact}\factlab{match:sig:vtx}{\cite{dks-clust-16}}
For any curve $P$ and any $\delta>0$, let $S$ be the $\delta$-signature of $P$.
Let $v_1,\dots,v_k$ denote the vertices of $S$. Let $r_i=[v_i-\eps,v_i+\eps]$,
for $1\leq i \leq k$ and for some value $\eps \in (0,\delta]$, be ranges
centered at the signature vertices. It holds for any curve $Q$ if
$\distFr{P}{Q}\leq \eps$, then $Q$ has a vertex in each range $r_i$, and such
that these vertices appear on $Q$ in the order
of $i$.  \end{fact}

%
%\paragraph{tight matchings}
%Given two curves $\tau_X$ and $\tau_Y$, consider a monotone path $f$ through
%the parametric space of $\tau_X$ and $\tau_Y$ consisting of two types of
%segments: (i) segments contained in the $0$-free space, and (ii) horizontal
%line segments contained in the $\delta$-free space. If $f$ exists, we say that
%$f$ is a \emph{tight matching} of width $\delta$ from $\tau_X$ to $\tau_Y$.
%Note the asymmetry in the definition.  Intuitively, tight matchings have the property that
%they match every point on $\tau_Y$ (vertical axis in the free space diagram) 
%to a point on $\tau_X$ (horizontal axis in the free space diagram) at distance zero, 
%but not necessarily the other way around. Technically, we have to ensure that the 
%matching is a bijection, but this is a non-problem.
%
%\begin{lemma}\lemlab{tight:matching:exists}
%Given a directed edge $e_Y$ and a curve $\tau_X$ which starts at the first
%endpoint of $e_Y$ and ends at the second endpoint of $e_Y$, if
%$\distFr{\tau_X}{e_Y}\leq \delta$, then there also exists a tight matching of
%width $\delta$. 
%\end{lemma}
%\begin{proof}
%TODO
%\end{proof}
% 
%\begin{figure}
%\centering
%\includegraphics{figs/tightmatchingex}
%\caption{Example of a tight matching between a one-dimensional polygonal curve and a line segment that shares endpoints with the curve.}
%\end{figure}
%
%
%\begin{lemma}\lemlab{tight:matching:chained} 
%Given three curves $\tau_1$, $\tau_2$ and $\tau_3$, such that there exists
%tight matchings of width $\delta$ from $\tau_1$ to $\tau_2$ and from $\tau_3$
%to $\tau_2$, then it holds that $\distFr{\tau_1}{\tau_3}\leq \delta$.
%\end{lemma}
%\begin{proof}
%TODO
%\end{proof}
%

\subsection{Analysis}

\begin{lemma}\lemlab{cfd:a1}
Let $P, Q \in \Curves{1}$ two curves with $m_1$ and $m_2$ points, respectively,
and let $m=\min\{m_1,m_2\}$. For any $\delta>0$, if $t$ is chosen uniformly
at random in $[0,1)^d$, then 
\[\Prob{{h^t_{\delta}(P)}={h^t_{\delta}(Q)}}{}\geq 1- \pth{2m\frac{ \distFr{P}{Q}}{\delta}},\]
\end{lemma}
\begin{proof}
Without loss of generality we assume that $m=m_1$. 
We would like to use a similar approach as in the proof of \lemref{dfd:a1}.
However instead of a discrete traversal and components, we now have to deal
with a continuous traversal of the curves. However, we can simulate the role of
components by considering the portion of the curve that lies in the vicinity of
a signature vertex. Concretely, let $\distFr{P}{Q}=\alpha$ 
and consider the $\alpha$-signature of $P$. By \factref{match:sig:vtx}, the
curve $Q$ needs to visit the $\alpha$-ranges around the signature vertices in
the order along $P$ (and it needs to do so with a vertex).  
Let $v_1,\dots,v_m'$ be the sequence of vertices of the $\alpha$-signature of $P$.
Let $A_i$ be the event that there exist two points $p,q \in
[v_i-\alpha,v_1+\alpha]$ which would be separated by the random shift (that is,
they would be snapped to different grid points). Since $t$ is uniformly random
in $[0,1)$, we have for $1 \leq i \leq m'$ that 
\[\Prob{A_i}{} \leq \frac{2\alpha}{\delta}.\]
In the event that none of the ranges are separated, it must be that the \Frechet 
distance of the two curves after snapping will be zero.
In this case, the second step, which removes redundant vertices, ensures
that also the sequence of vertices is the same.

Therefore, we have 
\begin{eqnarray*}
\Prob{{h^t_{\delta}(P)}={h^t_{\delta}(Q)}}{} \geq 1 - 
\Prob{\bigcup_{1\leq i\leq m'} A_i}{}   
 \geq 1 - \sum_{1\leq i\leq m'} \Prob{A_i}{}   
 \geq 1 - m\cdot \frac{2\alpha}{\delta}.
\end{eqnarray*}
Since we defined $\alpha$ as the distance $\distFr{P}{Q}$, the lemma follows.
\end{proof}

\begin{lemma}\lemlab{cfd:a2}
For any value of $\delta$ and for any $P,Q \in \Curves{1}$, if there exists a value of $t \in [0,1]^d$ such that 
$h^t_{\delta}(P)=h^t_{\delta}(Q)$, then it holds that $\distFr{P}{Q} \leq \delta.$
\end{lemma}

\begin{proof}
In the case that $h^t_{\delta}(P)=h^t_{\delta}(Q)$, it holds that $\distFr{h^t_{\delta}(P)}{h^t_{\delta}(Q)}= 0$.
Furthermore, the removal of redundant vertices does not change the \Frechet distance.
Since the snapping to the randomly shifted grid changes the position of each
vertex by at most $\delta/2$, we also have that $\distFr{P}{h^t_{\delta}(P)} \leq \delta/2$ and similarily 
$\distFr{Q}{h^t_{\delta}(Q)} \leq \delta/2$. By the triangle inequality,
\begin{eqnarray*}
\distFr{P}{Q} \leq \distFr{h^t_{\delta}(P)}{P} + \distFr{h^t_{\delta}(P)}{h^t_{\delta}(Q)} + \distFr{h^t_{\delta}(Q)}{Q} \leq \delta.
\end{eqnarray*}
\end{proof}

Using the above lemmas we obtain the same result as was stated in \thmref{basic:dfd} for the discrete \Frechet distance:
\begin{theorem}\thmlab{basic:cfd}
Let $P, Q \in \Curves{1}$ two curves with $m_1$ and $m_2$ points, respectively, and let $m=\min\{m_1,m_2\}$, $\delta= 4mr$ and  $c=4m$.
If $t$ is chosen uniformly at random in $[0,1)$, then it holds that: 
\begin{compactenum}[(i)]
\item if $\distFr{P}{Q} < r$, then $\Prob{h^t_{\delta}(P)=h^t_{\delta}(Q)}{} > \frac{1}{2}$
\item if $\distFr{P}{Q} > cr$, then $\Prob{h^t_{\delta}(P)=h^t_{\delta}(Q)}{} = 0,$
\end{compactenum}
\end{theorem}



%A corollary of the previous lemma is that if $\distFr{P}{Q} > \delta$, then $\Prob{h(P)=h(Q)}{\Hash}=0$.
%The above would be a $(r,cr,\frac{1}{2},0)$- sensitive LSH with linear approximation factor
% $c=O\pth{N\pth{P,\frac{3}{2}\delta}+N\pth{Q,\frac{3}{2}\delta}}$.

